Mind the Trade-off: Debiasing NLU Models without Degrading the In-distribution Performance

Models for natural language understanding (NLU) tasks often rely on the idiosyncratic biases of the dataset, which make them brittle against test cases outside the training distribution. Recently, several proposed debiasing methods are shown to be very effective in improving out-of-distribution performance. However, their improvements come at the expense of performance drop when models are evaluated on the in-distribution data, which contain examples with higher diversity. This seemingly inevitable trade-off may not tell us much about the changes in the reasoning and understanding capabilities of the resulting models on broader types of examples beyond the small subset represented in the out-of-distribution data. In this paper, we address this trade-off by introducing a novel debiasing method, called confidence regularization, which discourage models from exploiting biases while enabling them to receive enough incentive to learn from all the training examples. We evaluate our method on three NLU tasks and show that, in contrast to its predecessors, it improves the performance on out-of-distribution datasets (e.g., 7pp gain on HANS dataset) while maintaining the original in-distribution accuracy.

==> old_text.tex <==
% \begin{table}
%     \centering
%     \setlength{\tabcolsep}{3pt}
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l c c c c}
%         \toprule
%          \multirow{2}{*}{Method} & \multicolumn{2}{c}{MNLI-m} & \multicolumn{2}{c}{MNLI-mm} \\
%         & dev-hard & test-hard & dev-hard & test-hard \\
%         \midrule
%         BERT-base\textsubscript{ none} & 75.7 \footnotesize{$\pm$ 0.4} & 76.8 & 76.9 \footnotesize{$\pm$ 0.2} & 75.9\\
%         \midrule
%         Learned-mixin\textsubscript{ hypo} & \cellcolor{green(munsell)} 78.8 \footnotesize{$\pm$ 0.5} & \cellcolor{green(munsell)} 79.2 & \cellcolor{green(munsell)} 80.1 \footnotesize{$\pm$ 0.4} & \cellcolor{green(munsell)} 78.2\\ % seed 222
%         Product-of-expert\textsubscript{ hypo} & \cellcolor{green(munsell)} 78.3 \footnotesize{$\pm$ 0.4} & \cellcolor{green(munsell)} 79.8 & \cellcolor{green(munsell)} 79.2 \footnotesize{$\pm$ 0.4} & \cellcolor{green(munsell)} 78.7\\ % seed 222
%         \midrule
%         Regularized-conf\textsubscript{ hypo} & \cellcolor{grannysmithapple} 77.4 \footnotesize{$\pm$ 0.4} & \cellcolor{grannysmithapple}78.3 & \cellcolor{grannysmithapple}78.6 \footnotesize{$\pm$ 0.3} & \cellcolor{grannysmithapple}77.3\\ % seed 555
%         % Regularized-conf\textsubscript{ mix} & 77.02 & 77.90 & 78.51 & 77.30\\
%         \bottomrule
%     \end{tabular}}
%     \caption{Performance on hard data split based on the hypothesis only model. The test-hard result is obtained from online evaluation by \citet{Gururangan2018AnnotationAI}}
%     \label{tab:hypo}
%     \vspace{-4mm}
% \end{table}

% % We perform an extensive evaluation of our method on three benchmarks for each task: MNLI \cite{Williams2018ABC} for natural language inference, FEVER dataset \cite{Thorne2018TheFE} for fact verification and Quora Question Pairs for paraphrase identification. We use the existing \textit{challenge test sets} for each task that are designed to models' robustness against specific types of artifacts. The already identified artifacts of each task are used to determine the features for training the \textit{biased-models}.
% % the three tasks are formulated as a classification problem 
% % which artifacts that we consider and what evaluation data that we use

% % \paragraph{} We consider two strong debiasing baselines. The first one is the variant of \textit{product-of-expert} method \cite{Hinton2002TrainingPO} which is recently proposed by three concurrent work \cite{He2019UnlearnDB, Clark2019DontTT, Mahabadi2019SimpleBE}. The second baseline is the \textit{learned-mixin} method which is introduced by \citet{Clark2019DontTT} as an adaptive variant of \textit{product-of-expert}. During the training, learned-mixin allows the model to learn when to utilize the biased-model. When the model decide to use zero weight on the biased-model, then the loss incurred is the same as standard cross-entropy. We use the \textit{learned-mixin} added with entropy penalty term, which they show to perform consistently well across tasks given a proper hyperparameter. 

% % \subsection{Natural Language Inference (NLI)}
% % The goal of NLI task is to predict whether a \textit{premise} sentence is entailed by the \textit{hypothesis} sentence. We utilize MNLI dataset \cite{Williams2018ABC} which consist of text pairs from diverse set of domains. Each example has three possible labels: \textit{entailment}, \textit{neutral}, and \textit{contradiction}.

% % \paragraph{Detecting biased examples} We address two identified types of bias within the MNLI dataset: (1) \textit{hypothesis-only} bias (2) \textit{lexical-overlap} bias. Following the previous debiasing work, we train a biased-model to identify examples that exhibit either bias . Hypothesis-only bias is characterized by words in the hypothesis that are strongly associated with certain labels. To capture the hypothesis-only bias, we train an Infersent model which predicts the label using only hypothesis sentence as the input \cite{Poliak2018HypothesisOB}. 

% % Lexical-overlap bias, on the other hand, presents a structural cue that appear when the hypothesis is compared to the premise only on the surface level. To detect examples with \textit{lexical-overlap} bias, we train an MLP classifier using handcrafted-features as the biased-model. Following \citet{Clark2019DontTT} these handcrafted-features include (a) whether words in the hypothesis are completely overlap with words in the premise, (b) whether the hypothesis is the contiguous subsequence of the premise, (c) the percentage of words in the hypothesis that are also appear in the premise, (d) the mean of the minimum cosine distances between the embedding of words in the premise and the embedding of words in the hypothesis, (e) the max of the previously computed distances.\footnote{We include the details of the biased-model training in the appendix.}

% % \paragraph{Unbiased datasets} To evaluate model's utilization of hypothesis-only bias, we consider the \textit{hard} split of both development and test sets where examples cannot be predicted correctly by the hypothesis-only biased-model. \citet{Gururangan2018AnnotationAI} provides hard splits of MNLI test sets. We perform a similar procedure to create the same split on the dev sets. We use HANS (Heuristic Analysis for NLI Systems) \cite{McCoy2019RightFT} to evaluate how our method alleviates NLI models' reliance on the lexical-overlap bias. This dataset is introduced to expose models' tendency to predict \textit{entailment} when presented with premise and hypothesis pairs that are overlap. 

% % \paragraph{Results: in-distribution} Table \ref{tab:in_domain} shows in in-distribution performance of the debiasing methods compared to the baseline BERT. We observe the ability of our debiasing strategy in retaining the in-distribution performance while effectively improving the accuracy on the challenge test sets (as shown next). The learned-mixin is noticeably more sensitive to the choice of the biased-model, dropping up to 4 percentage point on the dev-matched set of MNLI.
% % table on the test submission results

% % \paragraph{Results: hypothesis-only bias} We show the results on table \ref{tab:hypo}. Our method obtains improvement that ranges from 1 to 2 percentage point on the 4 hard splits. We observe that both learned-mixin and product-of-expert gain higher improvement but at the cost of substantial in-distribution performance drop, as shown table \ref{tab:in_domain}.

% % \paragraph{Results: lexical-overlap bias} Table \ref{tab:hans_scores} shows the results on HANS dataset. We show that our method obtains 7 points improvement on the average score of HANS. Product-of-experts provides the similar gain but reduces the performance on the MNLI dev-match set by a substantial margin. We observe that Learned-mixin may have ignore the biased-model to retain the accuracy on the in-distribution data. Its mild improvement is contributed by the gain on the non-entailment examples in the constituent subset of HANS.

% % \subsection{Fact Verification}
% % We consider the FEVER dataset \cite{Thorne2018TheFE} to evaluate our method on the fact verification task. The dataset consist of pairs of claim and evidence sentences. The goal of the task is to make an assessment of whether the evidence sentence \textit{supports}, \textit{refutes}, or provides \textit{not enough information} about the validity of the given claim.\footnote{We use the train and dev split of the preprocessed FEVER data by \citet{schuster2019towards}}

% % \paragraph{Detecting biased examples} We address the \textit{claim-only} bias in FEVER dataset, which previously studied by \citet{schuster2019towards}. Their study find that specific n-grams in the claim sentences are strongly correlated with target labels. Similar to the \textit{hypothesis-only} bias in NLI task, we train a biased-model that predicts the label using only the claim as the input. 
% % \paragraph{Unbiased datasets} We evaluate on Symmetric test set \cite{schuster2019towards} which is designed to break FEVER models that make use of the indicative n-grams in the claim sentence. Since the size of the test set is small, we additionally use the newest version of the test set which add new test examples to the old one.

% % \paragraph{Results: in-distribution} The left most column of table \ref{tab:fever} shows the in-distribution performance on the existing dev set. We observe slight improvement over BERT baseline from our debiasing strategy. The example-reweighting strategy\footnote{also used by \citet{Mahabadi2019SimpleBE} and \citet{Clark2019DontTT}} used by \citet{schuster2019towards} is able to retain the in-distribution performance. Learned-mixin and product-of-expert sustain the worse in-distribution degradation, dropping almost 3 percentage point.

% % \paragraph{Results: claim-only bias} As shown by table \ref{tab:fever}, our debiasing strategy provides a comparable improvement on the two Symmetric test sets. We observe less variability of the improvement that our method provide despite the small size of the test sets.

% % \subsection{Quora Question Pairs (QQP)}
% % Quora Question Pairs present a task of detecting whether a pairs of questions is a paraphrase or semantically equivalent. The question pairs in the dataset are labeled as either \textit{duplicate} or \textit{not-duplicate}.

% % \paragraph{Detecting biased examples} The dataset is reported to contain several biases \cite{Zhang2019PAWSPA, zhang-etal-2019-selection}. We address the lexical overlap bias. We use the same biased-model as in HANS evaluation.

% % \paragraph{Unbiased datasets} We evaluate on PAWS (Paraphrase Adversaries from Word Scrambling) dataset \cite{Zhang2019PAWSPA} which consist of both paraphrase and non-paraphrase question pairs with high lexical overlap. We report separate scores for each duplicate and non-duplicate questions.

% % \paragraph{Results: in-distribution} Results are shown on table \ref{tab:qqp_paws}. We observe that all debiasing methods, including ours, sustain slight drop of performance in the in-distribution data of QQP. Our method shows the least performance drop on the duplicate questions examples. Learned-mixin notably decreases the performance on the duplicate examples up to 10\%. As shown later in the discussion, we demonstrate that the large portion of biased examples in QQP may lead to this degradation by all debiasing methods.

% % \paragraph{Results: lexical-overlap bias} As seen from table \ref{tab:qqp_paws}, the confidence-regularization method is able to improve the ability to detect \textit{non-duplicate} PAWS example by 10 percentage point. This comes with only a slight decrease of performance on the \textit{duplicate} examples. The two baseline methods, show stronger improvement on the \textit{non-duplicate} subsets of PAWS, although at the cost of substantial accuracy drop on the \textit{duplicate} questions counterpart. 

% % \paragraph{Augmenting QQP with PAWS} We observe that only around 20\% of QQP examples do not exhibit lexical-overlap bias. This may provide weak training signal for all debiasing methods that we consider. We therefore investigate whether the behavior of these methods changes as the proportion of unbiased examples in the dataset is increased. To this end, we split PAWS data into a training set which consist of 2500 examples and use the remaining 10K examples as a test set. We consider the product-of-expert method and the standard BERT baseline as a comparison to ours. On each method, we perform separate training runs using different fraction of the PAWS train split to augment QQP, and evaluate on the same PAWS test set. Figure \ref{fig:paws_augmented} shows the results.

% % We observe that while the augmentation with PAWS examples do not effect the in-distribution QQP performance, it gradually improves the three methods on the PAWS test set. The two debiasing methods are able to improve the performance further on top of the improvement that comes from the augmentation. We note that our method is the most effective when the entire 2500 unbiased examples are included in the training. It increase the non-duplicate accuracy up to 84.5\% while keeping the duplicate accuracy above 61\%. Produce-of-expert, on the other hand, drops the duplicate accuracy to 40\% to obtain the 93\% non-duplicate accuracy.

% % \subsection{Controlled Input Manipulation}
% % \ajie{Incomplete. Put more thoughts on why this analysis is important.} 
% % In this section, we investigate whether the debiased models are more sensitive to semantics changes in the input. To this end, we perform a controlled input manipulation, in which we measure the changes in model's prediction when the input is perturbed such that the meaning is changed. We consider two types of input perturbation: (1) nouns swapping (2) random verb word dropping. These perturbation either shift the meaning or result to non-sensical input. We measure the KL-divergence of output distribution before and after the perturbation.

% % under the shift of distribution 
% % we propose a bias-weighted scaling
% % incentivize to learn from the easy example in the right way
% % we refer to our model as confidence regularization

% % We introduce a variant of label smoothing technique \cite{Szegedy2015RethinkingTI}, in which the loss is computed with ``\textit{soft}'' target distributions, instead of hard targets from the dataset. We employ a distillation training \cite{Hinton2015DistillingTK} to produce ``\textit{soft}'' target labels that encodes a meaningful knowledge about the task. Next, we use a measure of example bias to scale down the target distribution, i.e., adjusting the ratio between labels' probability without changing the argmax. In order to quantify the weight of a bias, we train a \textit{biased-model}\footnote{we borrow the terminology used by \citet{He2019UnlearnDB}} to perform the task using only the biased surface features. Figure \ref{fig:method_illustration} illustrates an example of applying our debiasing strategy on the NLI task.

% % We use our method to train models for three semantic relationship identification tasks: textual entailment, fact verification, and duplicate questions detection. For each task, we perform an evaluation on the existing adversarial test sets to evaluate model's ability to generalize to out-of-distribution data. We observe that our approach provides a substantial improvement over the baseline model BERT \cite{devlin2018bert}, while maintaining or even improving the original in-distribution accuracy. 
% % % The latter aspect is especially important as it provides an advantage over previous debiasing methods \cite{He2019UnlearnDB, Clark2019DontTT, Cadne2019RUBiRU} which require a trade-off between the in-distribution performance and the robustness against the out-of-distribution data.

% % Our ablation study indicates that knowledge distillation alone does not improve the performance on the adversarial test sets. Additionally, applying bias-based example weights for label smoothing \cite{Szegedy2015RethinkingTI} brings adverse effect to model's performance in both in-distribution and adversarial scenario. We also observe that the effectiveness of our method is increased as more unbiased examples are added to the training data.
% % % the behavior

% % In summary, we make the following contributions in this paper: (1) We introduce a novel debiasing method which regularize model's confidence on biased training examples. (2) An emperical evaluations to compare our debiasing strategy against the baseline methods and to provide insights about their behavior across different scenarios. (3) We analyze the impact of each component in our strategy in mitigating bias and mantaining in-distribution performance.

% % This trade-off contradicts the intuition that the generalizable representations learned by a robust model should align well to both 
% % model should learn to correct for the right reason
% % this contradicts the intuition that ...
% % These methods work by limiting the training signal from the biased examples that are predicted well by the naive model, which can be seen as. 
% % While these methods are able to improve the out-of-distribution performance, 
% % these methods work by limiting the training signal from examples that are predicted well by the weak model. 
% % this improvement comes at the cost of the in-distribution performance. 
% % This trade-off is the result of the ensembling process which inherently limits the training signal from the biased examples to the model. 
% % This is especially not ideal because a debiasing process should learn a more generalizable representation from both \textit{biased} and \textit{unbiased} examples. 
% % This trade-off can be unfavourable in scenario 

% % we argue that we need to still able to learn from biased examples although in different way
% % general representation 
% % different way of using biased-examples -- other work reduce the contribution
% % in this paper we show that we can minimize this trade-off 

% % Due to their reliance on biased features, models often make incorrect predictions with high confidence in their output probability on such adversarial examples \cite{nguyen2015deep, Feng2018PathologiesON}. 
% % As argued by \citet{Lewis2019GenerativeQA}, this phenomenon can be partially explained by the loss function based on maximum likelihood estimation, which saturates when simple correlations allows an example to be predicted confidently. Models therefore overfit to the biased features as there is no further incentive to learn the underlying semantics of an example. Consequently, model may be insensitive to changes in semantics when the surface feature is retained.

% \begin{table}
%     \centering
%     \setlength{\tabcolsep}{3pt}
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l c c | c c | c c}
%         \toprule
%           \multirow{3}{*}{Dataset / bias} & \multicolumn{2}{P{2cm}}{product-of-expert} & \multicolumn{2}{|P{2cm}|}{learned-mixin} & \multicolumn{2}{P{2cm}}{\textbf{conf-reg (our)}}\\
%         % \midrule
%          & \textit{in} & \textit{out} & \textit{in} & \textit{out} & \textit{in} & \textit{out} \\
%         \midrule
%         MNLI \textsubscript{lexical-overlap} & \FancyDownArrowMedium & \FancyUpArrowHeavy & \FancyDownArrowNeutral & \FancyUpArrowLight & \FancyUpArrowLight & \FancyUpArrowHeavy \\
%         MNLI \textsubscript{hypothesis-only} & \FancyDownArrowMedium & \FancyUpArrowMedium & \FancyDownArrowHeavy & \FancyUpArrowHeavy & \FancyUpArrowLight & \FancyUpArrowMedium \\
%         Fever \textsubscript{claim-only} & \FancyDownArrowMedium & \FancyUpArrowMedium & \FancyDownArrowHeavy & \FancyUpArrowLight & \FancyUpArrowHeavy & \FancyUpArrowMedium \\
%         QQP \textsubscript{lexical-overlap} & \FancyDownArrowNeutral & \FancyUpArrowHeavy & \FancyDownArrowNeutral & \FancyUpArrowHeavy & \FancyDownArrowNeutral & \FancyUpArrowLight \\
%         \midrule
%         Calibration & \multicolumn{2}{c}{\FancyUpArrowNeutral} & \multicolumn{2}{|c|}{\FancyUpArrowNeutral} & \multicolumn{2}{c}{\FancyUpArrowLight} \\
%         % Regularized-conf\textsubscript{ mix} & 84.11 & - & 84.91 & -\\
%         \bottomrule
%     \end{tabular}}
%     \caption{Comparison of our confidence regularization method against other state-of-the-art debiasing methods. The left most column shows the evaluated datasets along with their biased feature. The two colored arrows in each cell indicate the changes in in-distribution and out-of-distribution performance respectively.}
%     \label{tab:comparison}
%     \vspace{-4mm}
% \end{table}

% \begin{table*}
%     \small
%     \begin{center}
%     \setlength{\tabcolsep}{3pt}
%     % \resizebox{\textwidth}{!}{%
%      \begin{tabular}{l c c c c c} 
%      \midrule
%      \multirow{2}{*}{Method} & \multirow{2}{*}{MNLI\textsubscript{ dev}} & \multicolumn{2}{c}{lexical} & \multicolumn{2}{c}{subseq} & \multicolumn{2}{c}{const} & \multirow{2}{*}{Avg} \\
%      & & E & $\neg$E & E & $\neg$E & E & $\neg$E \\
%      \midrule
%      BERT-base & 84.4 \tiny{$\pm$ 0.1} & 95.6 \tiny{$\pm$ 1.6} & 54.6 \tiny{$\pm$ 11.5} & 99.5 \tiny{$\pm$ 0.4} & 8.8 \tiny{$\pm$ 4.1} & 99.4 \tiny{$\pm$ 1.9} & 14.8 \tiny{$\pm$ 1.9} & 62.1 \tiny{$\pm$ 2.1}\\
%      \midrule
     
%      Learned-mixin\textsubscript{ hans} & \cellcolor{ghostwhite} 84.0 \tiny{$\pm$ 0.2} & 94.9 \tiny{$\pm$ 0.1} & 53.5 \tiny{$\pm$ 14.7} & 99.5 \tiny{$\pm$ 0.3} & 8.2 \tiny{$\pm$ 1.4} & 98.9 \tiny{$\pm$ 0.4} & 24.1 \tiny{$\pm$ 1.2} & \cellcolor{ghostwhite} 63.4 \tiny{$\pm$ 2.4}\\
     
%      Product-of-expert\textsubscript{ hans} & \cellcolor{pastelred} 82.2 \tiny{$\pm$ 0.8} & 64.6 \tiny{$\pm$ 9.7} & 81.1 \tiny{$\pm$ 3.9} & 77.3 \tiny{$\pm$ 12.8} & 53.3 \tiny{$\pm$ 17.1} & 74.8 \tiny{$\pm$ 11.1} & 64.3 \tiny{$\pm$ 9.1} & \cellcolor{green(pigment)} 69.2 \tiny{$\pm$ 2.6}\\
     
%      \midrule
%      \textbf{Regularized-conf\textsubscript{ hans}} & \cellcolor{ghostwhite} 84.3 \tiny{$\pm$ 0.1} & 68.5 \tiny{$\pm$ 6.5} & 78.2 \tiny{$\pm$ 3.7} & 84.5 \tiny{$\pm$ 5.9} & 48.5 \tiny{$\pm$ 7.1} & 84.7 \tiny{$\pm$ 5.4} & 49.6 \tiny{$\pm$ 3.7} & \cellcolor{green(pigment)} 69.1 \tiny{$\pm$ 1.2}\\
%     %  Regularized-conf\textsubscript{ mix} & 76.56 & 79.22 & 89.44 & 38.22 & 87.72 & 44.02 & 69.19\\
%      \bottomrule
%     \end{tabular}%}
%     \end{center}
%     \caption{Fine-grained scores on HANS evaluation benchmark. The probability of non-entailment label is obtained by taking the max of neutral and contradiction probabilities.}
%     \label{tab:hans_scores}
%     \vspace{-4mm}
% \end{table*}
